DynInt: Dynamic Interaction Modeling for Large-scale Click-Through Rate Prediction

Learning feature interactions is the key to success for the large-scale CTR prediction in Ads ranking and recommender systems. In industry, deep neural network-based models are widely adopted for modeling such problems. Researchers proposed various neural network architectures for searching and modeling the feature interactions in an end-to-end fashion. However, most methods only learn static feature interactions and have not fully leveraged deep CTR models' representation capacity. In this paper, we propose a new model: DynInt. By extending Polynomial-Interaction-Network (PIN), which learns higher-order interactions recursively to be dynamic and data-dependent, DynInt further derived two modes for modeling dynamic higher-order interactions: dynamic activation and dynamic parameter. In dynamic activation mode, we adaptively adjust the strength of learned interactions by instance-aware activation gating networks. In dynamic parameter mode, we re-parameterize the parameters by different formulations and dynamically generate the parameters by instance-aware parameter generation networks. Through instance-aware gating mechanism and dynamic parameter generation, we enable the PIN to model dynamic interaction for potential industry applications. We implement the proposed model and evaluate the model performance on real-world datasets. Extensive experiment results demonstrate the efficiency and effectiveness of DynInt over state-of-the-art models.

==> backlog.tex <==
\subsection{Embedding Layer}

In large-scale recommendation system, inputs include both continuous features and categorical features. Categorical features are often directly encoded by one-hot encoding, which results in an excessively high-dimensional and sparse feature space. 
Suppose we have $F$ fields. In our feature preprocessing step, we bucketize all the continuous features to equal frequency bins, then embed the bucketized continuous features and categorical features to same latent space $R^K$,
\begin{equation*}
	\mathbf{x}^{e}_{f} = \mathbf{x}^{o}_{f}\mathbf{V}_{f},
\end{equation*}
where $\mathbf{x}^{e}_{f}=[x_{f,1},x_{f,2},\cdots,x_{f,K}]$, $x_{f,k}$ is the $k$-th bit of the $f$-th field of the embedding feature map, $\mathbf{V}_f$ is an embedding matrix for field $f$, and $\mathbf{x}^{o}_f$ is a one-hot vector. Lastly, we stack $F$ embedding vectors and obtain an $F$-by-$K$ input feature map $X_0$:
\begin{equation*}
	X_0=\begin{bmatrix}
		\mathbf{x}^{e}_{1} \\
		\mathbf{x}^{e}_{2} \\
		\vdots \\
		\mathbf{x}^{e}_{F}
	\end{bmatrix}
\end{equation*}

\subsection{Polynomial Interaction Network}
Consider a $l$-th order polynomial with $f$ variables of the following form:
\begin{equation} \label{equ:poly}
\begin{aligned}
\Pi_{j=1}^{l}(\sum_{i=1}^f a_{ij}x_{i}+b_{j}).
\end{aligned}
\end{equation}
This polynomial contains all possible multiplicative combinations of $x_i$'s with order less than or equal to $l$ and has an iterative form:
\begin{equation} \label{equ:poly_iterative}
\begin{aligned}
F^{(l-1)}(x_1,\cdots, x_f)(\sum_{i=1}^f a_{il}x_{i}+b_{l})
\end{aligned}
\end{equation}
where $F^{(l-1)}(x_1,\cdots, x_f)=\Pi_{j=1}^{l-1}(\sum_{i=1}^f a_{ij}x_{i}+b_{j})$. Motivated by the iterative form, we propose polynomial interaction network defined by the following formula:
\begin{equation}\label{interaction-layer}
\begin{aligned}
X_l & = f(W_{l-1}, X_{l-1}, X_0) + X_{l-1} \\
& = X_{l-1} \circ (W_{l-1}X_0) + X_{l-1} \\
 & = X_{l-1} \circ [W_{l-1}X_0 + \mathbf{1}] \\
\end{aligned}
\end{equation}
where $\circ$ denotes the Hadamard product. For instance, $[a_{i,j}]_{m\times n}\circ [b_{i,j}]_{m\times n} = [a_{i,j}b_{i,j}]_{m\times n}$. $W_{l-1}\in R^{F\times F}$ and $\mathbf{1}\in R^{F\times K}$ with all entries are equal to one. $X_{l-1}, X_l \in R^{F\times K}$ are the output matrices of ($l$-1)-th and $l$-th interaction layer. Like \eqref{equ:poly}, the $l$-th PIN layer's output is the weighted sum of all vector-wise feature interactions of order less than or equal to $l$.

The architecture of the polynomial interaction network is motivated by the following aspects.

First, the polynomial interaction network has a recursive structure. The outputs of the current layer are built upon the previous layer's outputs and the first order feature map, ensuring that higher-order feature interactions are based on lower-order feature interactions from previous layers.

Second, we use the Hadamard product to model the explicit vector-wise interaction, which brings us more flexibility in crossing the bits of each dimension in shared latent space and preserves more information of each degree of feature interactions.

Third, we build a field aggregation layer $Agg^{(l)}(X)=W_{l}X$ which combines the feature map at the vector-wise level using a linear transformation $W_{l}$. Each vector of the field aggregation feature map can be viewed as a combinatorial feature vector constructed by the weighted sum of the input feature map. Then we take the Hadamard product of the output of the previous layer and field aggregation feature map for this layer. This operation allows us to explore all possible $l$-th order polynomial feature interactions based on existing ($l$-1)-th order feature interactions.

Last, we utilize residual connections~\cite{he2016deep,veit2016residual} in the polynomial interaction network, allowing a different degree of vector-wise polynomial feature interactions to be combined, including the first feature map. Since the polynomial interaction layer's outputs contain all degree of feature interactions, the skipped connection enable next polynomial interaction layer to focus on searching useful higher-order feature interactions while complementing lower-order feature interactions.
\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth]{figure/pin_layer.png}
	\caption{Details of PIN layer}
	\medskip
    \small
    The aggregation layer is defined by $Agg^{(l)}(X_0) = W_lX_0$. The PIN takes the Hadamard product of the aggregated 1st-order feature map and the output of the previous PIN layer to generate the higher order vector-wise interaction.
\end{figure}
As the number of layer increases, the degree of the polynomial feature interactions increases. The recurrent architecture of the proposed polynomial interaction network enables to bound the degree of polynomial feature interactions.

\subsection{Subspace-crossing Mechanism}

The Polynomial Interaction Network (PIN) models the vector-wise interactions. However, PIN does not learn the bit-wise interaction in the shared latent embedding space. In order to cross the bits of different embedding dimensions, we propose the subspace-crossing mechanism which allows xDeepInt to learn the bit-wise interactions. Suppose we split the embedding space into $h$ sub-spaces, the input feature map $X_{0}$ is then represented by $h$ sub-matrices as follow:
\begin{equation}
\begin{aligned}
X_0  &  = [X_{0,1}, X_{0,2}, \cdots, X_{0, h}] \\
\end{aligned}
\end{equation}
where $X_{0,i}\in R^{F\times K/ h}$ and $i=1,2\cdots,h$. Next, we stack all sub-matrices at the field dimension and construct a stacked input feature map $X_{0}^{'}\in R^{(F*h)\times (K/h)}$.
\begin{equation}\label{stacked_feature_map}
\begin{aligned}
X_{0}^{'} & = \begin{bmatrix}
X_{0,1} \\
X_{0,2} \\
\vdots \\
X_{0,h}
\end{bmatrix},
\end{aligned}
\end{equation}
where $X_{0,j}\in R^{F\times (K/h)}$ and $h$ denotes the number of sub-spaces. By splitting the embedding vector of each field to $h$ sub-vectors and stacking them together, we can align bits of different embedding dimension and create the vector-wise interactions on stacked sub-embeddings.
\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figure/subspace_crossing.png}
	\caption{Subspace-crossing mechanism}
\end{figure}
Accordingly, we feed $X_{0}^{'}$ into the Polynomial Interaction Network (PIN):
\begin{equation}
\begin{aligned}
X_1^{'}  & = X_0
^{'}\circ [W_{0}^{'}X_0^{'} + \mathbf{1}] \\
& \vdots\\
X_l^{'}  & = X_{l-1}^{'} \circ [W_{l-1}^{'}X_0^{'}+ \mathbf{1}] \\
\end{aligned}
\end{equation}
where $W_{l}^{'} \in R^{(F*h)\times (F*h)}$, $\mathbf{1}\in R^{(F*h)\times (K/h)}$ and $X_{l}^{'} \in R^{(F*h)\times (K/h)}$. 

The field aggregation of feature map and the multiplicative interactions building by Hadamard product are both of the vector-wise level in vanilla PIN layers. The subspace-crossing mechanism enhanced PIN takes the $h$ aligned subspaces as input, so that encouraging the PIN to capture the explicit bit-wise interaction by crossing features of the difference subspaces. The number of subspaces $h$ controls the complexity of bit-wise interactions. Larger $h$ helps the model to learn more complex feature interactions.

\subsection{Output Layer}
The output of Polynomial Interaction Network is a feature map that consists of different degree of feature interactions, including raw input feature map reserved by residual connections and higher-order feature interactions learned by PIN. For the final prediction, we merely use formula as follows:
\begin{equation}
\begin{aligned}
\hat{y} & = \sigma\big((W_{out}X_{l} + b\mathbf{1}^T)\mathbf{1} \big)
\end{aligned}
\end{equation}
where $\sigma$ is the sigmoid function, $W_{out}\in R^{1\times F}$ is a feature map aggregation vector that linearly combines all the features in the feature map, $\mathbf{1}\in R^K$ and $b\in R$ is the bias.

\subsection{Optimization and Regularization}
For optimization, we use Group Lasso Follow The Regularized Leader (G-FTRL)~\cite{ni2019feature} as the optimizer for the embedding layers for feature selection, and Follow The Regularized Leader (FTRL)~\cite{mcmahan2013ad} as the optimizer for the PIN layers for interaction selection.

Group lasso FTRL regularizes the entire embedding vector of insignificant features in each field to exactly zero, which essentially conducts feature selection and brings more training efficiency for industrial settings. The group lasso regularization is applied prior to the subspace splitting mechanism such that feature selection is consistent between each subspaces.

FTRL regularizes the single elements of weight kernel in PIN layers to exactly zero, which excludes insignificant feature interactions and regularizes the complexity of the model.

This optimization strategy takes advantages of the properties of the different optimizers and achieves row-wise sparsity and element-wise sparsity at embedding table and weight kernel respectively. Therefore, it improves generalization ability and efficiency for both training and serving. It also plays an important role in model compression.


\begin{figure}[t]
	\centering
	\includegraphics[width=0.4\textwidth]{figure/GroupLassoFTRL.png}
	\caption{Group Lasso FTRL v.s. FTRL}
	\medskip
    \small
    The Group Lasso FTRL regularizes the embedding table with group-wise sparsity. FTRL regularizes the weight kernels of PIN layer with element-wise sparsity.
\end{figure}

\subsection{Training}
The loss function we use is Log Loss,
\begin{align}
	\resizebox{.875\hsize}{!}{$\mbox{LogLoss}=
		-\dfrac{1}{N}\sum^{N}_{i=1}(y_{i}log(\hat{y}_{i})+(1-y_{i})log(1-\hat{y}_{i}))$},
\end{align}
where $y_i$ is the true label and $\hat{y}_{i}$ is the estimated click through rate. $N$ is the total number of training examples.


\subsection{Difference Between PIN and DCN}
PIN and DCN both have an iterative form. However, the two network architectures are quite different in extracting feature interactions.
\begin{equation}\label{DCN}
\begin{aligned}
x_l & = f_{DCN}(x_{l-1}, w_{l-1}, b_{l-1}) \\
& = x_0x_{l-1}^Tw_{l-1} + b_{l-1} + x_{l-1}
\end{aligned}
\end{equation}
For DCN, feature map are flattened and concatenated as a single vector. All higher order bit-wise interactions are firstly constructed by the term $x_0x_{l-1}^T$, and then aggregated by a linear regression for next layer. This structure results in a special format of the output. As discussed in \cite{lian2018xdeepfm}, the output the DCN layer is a scalar multiple of $x_0$. \cite{lian2018xdeepfm} also pointed out the downsides: 1) the output of DCN is in a special form, with each hidden layer is a scalar multiple of $x_0$ and thus limits expressive power; 2) interactions only come in a bit-wise fashion.

PIN constructs vector-wise feature interaction using Hadamard product, which preserve the information at vector-wise level. In order to allow different fields to cross at vector level, PIN firstly aggregates the input feature map by a linear transformation $W_{l-1}X_0$ for each iterative PIN layer and build interactions by term $X_{l-1} \circ W_{l-1}X_0$. Accordingly, PIN keeps the vector-wise structure of feature interactions and does not limit the output to a scalar multiple of $X_0$. Moreover, each PIN layer is directly connected with input feature map $X_0$, which improves model trainability. We also prove PIN's polynomial approximation property in later section.


\subsection{xDeepInt Analysis}

In this section, we analyze polynomial approximation property of the proposed xDeepInt model. We consider an xDeepInt model with $l$ PIN layers, a subspace crossing mechanism with $h$ subspaces and $F$ input feature with the same embedding size $K$.
\subsubsection{Polynomial Approximation}
In order to understand how PIN exploits the vector-wise interactions, we examine the polynomial approximation properties of PIN. Let $\mathbf{X}^{(0)} \in R^{F \times K}$ be the embedded feature vector with $\mathbf{x}_i = [x_{i1},\cdots,x_{iK}]$ being the $i$-th row. $\mathbf{x}_{i}^{(l)}=[x_{i1}^{(l)},\cdots,x_{iK}^{(l)}]$ is the $i$-th row of the output of $l$-th layer. Then, $x_{ik}^{(l)}$ has the following explicit form:
\begin{align}
	x_{ik}^{(l)}= x_{ik}^{(0)} \prod_{r=0}^{l-1}(\sum_{i=1}^Fw^{(r)}_{ij}x_{jk}^{(0)}+1), \text{for } k=1,\cdots, K
\end{align}
where $W^{(r)}=[w^{(r)}_{ij}]_{1\leq i,j \leq F}$ is the weight matrix at $r$-th PIN layer. The product $\prod_{r=0}^{l-1}(\sum_{i=1}^Fw^{(r)}_{ij}x_{jk}^{(0)}+1)$ is the weighted sum of all possible crossed terms of the embbeded input at the $k$-th bit having order less than or equal to $l-1$. Thus, $x_{ik}^{(l)}$ is the weighted sum of all crossed terms that contains $x_{ik}^{(0)}$ and has the order less than or equal to $l$.

For the bit-wise interaction modeled by subspace-crossing mechanism, we consider the case where the number of subspaces equals to the embedding size $K$. In this extreme case, each row of $W_0'X_0'$ is a weighted sum of all bits in all fields. This design allows the combination of embedded features at different bits. To be more explicit, we consider the stacked input feature map with $h=K$
\begin{equation}
	\begin{aligned}
		X_{0}^{'} & = \begin{bmatrix}
			X_{0,1} \\
			X_{0,2} \\
			\vdots \\
			X_{0,K}
		\end{bmatrix},
	\end{aligned}
\end{equation}
where $X_{0,i}=\begin{bmatrix}
x^{(0)}_{i,1} \\
x^{(0)}_{i,2} \\
\vdots \\
x^{(0)}_{i,F}
\end{bmatrix}\in R^F$ .The weight matrix $W'_0$ is given by
\begin{equation}
	\begin{aligned}
		W'_0= \begin{bmatrix}
			w^{(0)}_{1,1} & w^{(0)}_{1,2} & \cdots &  w^{(0)}_{1,K} & w^{(0)}_{1, K+1} & \cdots & w^{(0)}_{1, FK}\\
			\vdots & \vdots & \ddots & \vdots & \vdots &  \ddots & \vdots \\
			w^{(0)}_{FK,1} & w^{(0)}_{FK,2} & \cdots &  w^{(0)}_{FK,K} & w^{(0)}_{FK, K+1} & \cdots & w^{(0)}_{FK, FK}
		\end{bmatrix} \in R^{FK \times FK}.
	\end{aligned}
\end{equation}
Thus, the $k$-th row of $W'_0X'_0 + 1$ has the following form:
\begin{equation}
	\sum_{i=1}^F\sum_{j=1}^Kw^{(0)}_{k,(i-1)K+j}x_{i,j} + 1.
\end{equation}
This is a linear combination of bits in all fields, which allows the PIN exploit all crossing of the feature map at bit-wise level. For example, the $[(i-1)K+j]$-th row of $X'_l$ is given by
\begin{equation}
	x^{(l)}_{i,j}= x^{(0)}_{i,j}\prod_{r=0}^{l-1}\sum_{i=1}^F\sum_{j=1}^Kw^{(r)}_{k,(i-1)K+j}x_{i,j} + 1
\end{equation}
$x^{(l)}_{i,j}$ is the weighted sum of all crossed terms that contains $x^{(0)}_{i,j}$ and has the order less than or equal to $l$.

\subsubsection{Time Complexity}
The cost of computing feature maps $W_{l-1}X$ at $l$-th PIN layer is $\mathcal{O}(h F^2 K)$. For a $L$-layers xDeepInt model, the total cost of feature maps is $\mathcal{O}(L h F^2 K)$. The additional cost is from the Hadamard product and residual connection, which is $\mathcal{O}(L F K)$. In practice, $h$ is not too large. Hence, the total time complexity mainly relies on the number of fields $F$ and embedding size $K$. For an $L$ layers DNN with each layer has $D_k$ hidden nodes, the time complexity is $\mathcal{O}(FK \times D_1 \times D_2 + \sum_{k=2}^{L-1} D_{k-1}D_kD_{k+1})$. The time complexity of xDeepInt relies on the number of subspaces. Therefore, xDeepInt has higher time complexity than DNN when modelling higher degrees of bit-wise interactions.

\subsubsection{Space Complexity}
The embedding layer contains $\sum_{f=1}^F K \times C_f$ parameters, where $C_f$ is the cardinality of $f$-th field. The output layer aggregates the feature map at the last PIN layer. Hence, the output layers require $F + 1$ parameters. The subspace crossing mechanism needs $h^2\times F^2$ parameters at each PIN layer, which is the exact size of the weight matrix $W'_r$ with $0\leq r \leq l-1$.  There are $(K/h) \times k' + h^2\times F^2 \times l$ parameters in $l$ PIN layers. Usually, we will pick a small $h$ to control the model complexity and $k'$ is comparable to $K$. Accordingly, the overall complexity of the xDeepInt is approximate $O(h^2\times F^2\times l)$, which is affected by the embedding size $K$ heavily. A plain $L$ layers DNN with each layer has $D_k$ hidden nodes requires $FK \times D_1 + \sum_{k=2}^{L} D_{k-1}D_{k}$ parameters. The complexity mainly depends on the embedding size and the number of hidden nodes at each layer. To reduce the space complexity of xDeepInt, we can apply the method introduced in~\cite{lian2018xdeepfm}. The space complexity of the model can be further reduced by exploiting a $L$-order decomposition and replace the weight matrix $W'_r$ with two low-rank matrices.

